Estimation and Recovery of a Planted Dense Subgraph from a Single Network Cascade

We study the inference of a planted dense component in a sparse random graph from a single spreading process. The graph has an Erd\H{o}s-R\'enyi background with edge probability $p_n$ and contains a planted dense component of size $n^{\alpha}$, with $\alpha > 1/2$, whose internal edge density $\xi>0$ is constant. The edge set is unobserved; the data only consist of the successive infection times from a single realization of a continuous-time SI process with independent and exponentially distributed transmission times. We show that the planted dense component leaves a detectable signature in the spreading process: after the exploration enters the dense component, it undergoes a short phase of accelerated growth. By analyzing this phase, we localize its onset and endpoint. These localization results yield consistent estimators of the component-size exponent $\alpha$, the background edge density $p_n$, and the internal edge density $\xi$ from the infection times alone. When the identities of the infected vertices are also observed, we further establish consistent recovery of the planted dense component.

==> header.tex <==
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{epsf}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage[dvipsnames]{xcolor}

\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm}

\usepackage[utf8]{inputenc}
\usepackage[colorlinks=true, allcolors=blue]{hyperref}
\usepackage[authoryear]{natbib}
\usepackage{appendix}

\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\newsavebox{\bigimage}
\usepackage{multirow}
\usepackage{float}
\usepackage[nodisplayskipstretch]{setspace} 
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
%\usepackage{bm}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage{pifont}%
%\RequirePackage{algorithm}
%\RequirePackage{algorithmic}
\RequirePackage{forloop}
\RequirePackage{url}




\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

%\newtheorem{definition}{Definition}
%\newtheorem{assumption}{Assumption}
\newtheorem{remark}[theorem]{Remark}
%\newtheorem{example}{Example}
%\newtheorem{property}{Property}
%\newtheorem{condition}{Condition}


\newcommand{\independent}{\perp\mkern-9.5mu\perp}
\newcommand{\notindependent}{\centernot{\independent}}



